A Deterministic Hitting-Time Moment Approach to Seed-set Expansion over a Graph

We introduce HITMIX, a new technique for network seed-set expansion, i.e., the problem of identifying a set of graph vertices related to a given seed-set of vertices. We use the moments of the graph's hitting-time distribution to quantify the relationship of each non-seed vertex to the seed-set. This involves a deterministic calculation for the hitting-time moments that is scalable in the number of graph edges and so avoids directly sampling a Markov chain over the graph. The moments are used to fit a mixture model to estimate the probability that each non-seed vertex should be grouped with the seed set. This membership probability enables us to sort the non-seeds and threshold in a statistically-justified way. To the best of our knowledge, HITMIX is the first full statistical model for seed-set expansion that can give vertex-level membership probabilities. While HITMIX is a global method, its linear computation complexity in practice enables computations on large graphs. We have a high-performance implementation, and we present computational results on stochastic blockmodels and a small-world network from the SNAP repository. The state of the art in this problem is a collection of recently developed local methods, and we show that distinct advantages in solution quality are available if our global method can be used. In practice, we expect to be able to run HITMIX if the graph can be stored in memory.

==> notation-fund-rel.tex <==
\section{Notation and some fundamental relationships} \label{sec:notation}

Let $e_i$ and $e_i^T$ denote the $i$-th column and row, respectively, of the identity matrix.
The former is a ``column'' vector while the latter is a ``row'' vector. This notation is best illustrated by displaying the matrix
\[
I_n = \begin{pmatrix}
      1 & 0 & \cdots & 0 \vspace{.5ex} \\
      0 & 1 & \cdots & 0 \\
      \vdots & \vdots & \ddots & 0 \vspace{.5ex} \\
      0 & 0 & \cdots & 1 \\
    \end{pmatrix} = \begin{pmatrix}
                      e_1 & e_2 & \cdots & e_n \\
                    \end{pmatrix} = \begin{pmatrix}
                                      e^T_1 \vspace{.5ex} \\
                                      e^T_2 \\
                                      \vdots \vspace{.5ex}\\
                                      e^T_n \\
                                    \end{pmatrix}\,.
\]
The subscript $n$ is often omitted given the context of the analysis.
  Post-multiplication of a matrix $B \in \mathbb{R}^{m \times n}$ by $e_j$, or $Be_j$, selects the $j$-the column of a matrix and, pre-multiplication of a matrix $B$ by $e^T_i$ , or $e^T_i M$, selects the $i$-th row of $B$. We also define
\begin{equation} \label{vector-e}
  e \coloneqq \sum_{i=1}^n e_i = \begin{pmatrix}
                            1 & 1 & \cdots & 1 \\
                          \end{pmatrix}^T
  \,.
\end{equation}
%
Suppose that $\Omega = \{ i_1, \ldots, i_j\}$ is a collection of non-repeating integers satisfying $1\leq i_k \leq n$ for $k=1,\ldots, j$.
Let
\begin{equation} \label{def-Pi}
\Pi_\Omega \coloneqq  \begin{pmatrix}
                      e_{i_i} & \cdots & e_{i_j}
                     \end{pmatrix}  \in \mathbb{R}^{n\times j}
\end{equation}
be the matrix that results from retaining the $\Omega$ columns of the identity matrix of order $n$. When $\Omega = \{i_1\}$, we denote $ \Pi_\Omega = \Pi_{ \{i_1\} } = \Pi_{i_1} = e_{i_1}$ for ease of notation. Given a vector $f \in \mathbb{R}^n$ the two vectors
\[
\Pi_\Omega^T f \in \mathbb{R}^{j}\,, \text{ and } \Pi_\Omega \Pi_\Omega^T f \in \mathbb{R}^{n}\,
\]
remove and replace by zero the $\Omega$ components of $f$, respectively. If $\Omega^c$ denotes the complement of $\Omega$, then
\[
\begin{pmatrix} \Pi_\Omega & \Pi_{\Omega^c}\end{pmatrix}
\]
is a permutation of $I=I_n$. We also see that the choice
\begin{equation} \label{def-Omega_i}
\Omega_i \coloneqq \{1,2,\ldots,n\}\setminus \{i\}\,,
\end{equation}
i.e., $\Omega_i$ is the collection of the first $n$ positive integers except for $i$,  implies that
\[
\Pi_{i^c}^T B \Pi_{j^c} = \Pi_{\Omega_i}^T B \Pi_{\Omega_j}
\]
is the submatrix of $B$ that results when the $i$-th row and $j$-th column of $B$ are removed. The above demonstrates that $\Pi_\Omega$ and $\Pi_\Omega^T$ function as prolongation and restriction matrices, respectively. The former matrix embeds a vector in $\mathbb{R}^j$ to $\mathbb{R}^n$ while the latter matrix performs the dual operation, i.e.,
$\Pi_\Omega^T \colon\mathbb{R}^n \to \mathbb{R}^j$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% I believe we can follow the example of Palacios and avoid using the concept of
% boundaries to define the key equations for moments.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The following definition defines the important concept of the boundary of a collection of vertices in terms of the vertices adjacent to the vertices in the collection.
%
%\begin{definition}
%Let $\Omega = \{ i_1, \ldots, i_j\}$ be a collection of non-repeating vertex indices where $1\leq j \leq n$. The boundary $\partial \Omega$ of $\Omega$ is defined as
%\[
%\partial \Omega : = \big(\bigcup_{j\in \Omega} \partial \{j \} \big)\setminus \Omega\,,
%\]
%where $\partial \{j \}$ denotes the set of neighbors for the vertex $j$.
%\end{definition}
%
%Recall that $\Omega^c$ denotes the complement of $\Omega$; then we see that $\partial \Omega \subseteq \Omega^c$ so that the decomposition of the vertices of a graph is
%\begin{equation} \label{eq:graph-decomp}
%\Omega \cup \partial \Omega \cup \big( \Omega^c \setminus \partial \Omega\big)\,.
%\end{equation}
%%The definition then implies that $\Omega \cap \Omega^c \setminus \partial \Omega = \emptyset$, i.e., there are no edges between $\Omega$ and $\Omega^c \setminus \partial \Omega $ so that $\Omega$ and $ \partial \Omega $ are disconnected.

\begin{definition}\label{def:graph-diff}
The combinatorial graph Laplacian is given by
\[
L\coloneqq D-A \in \mathbb{R}^{n \times n}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Question: Here, should we specify A and D in R_+^{nxn}, not just R^{nxn}?
% Also, we should specify that we can handle non-integer values in A (and hence D).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $D \in \mathbb{R}^{n\times n}$ is a diagonal matrix containing the degree of each vertex, and $A \in \mathbb{R}^{n\times n}$ is the adjacency matrix for a connected  graph with $n$ vertices containing possible multiple edges (including self-loops).
\end{definition}
For the remainder of our document, we assume that the graph is connected or, equivalently, the nullspace of $L$ is one dimensional, i.e., only contains only constant vectors.


==> tab/sbmSizeTab.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Tue Apr 28 09:40:55 2020
\begin{table}[ht]
\centering
\begin{tabular}{ll|cc}
  \hline
Method & Size of Non-Goal Block & Median $F_1$ & Median ARI \\ 
  \hline
HITMIX & 1000 & 1.00 (0.99, 1.00) & 0.99 (0.97, 1.00) \\ 
  HITMIX & 3000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  HITMIX & 5000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  CRD & 1000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  CRD & 3000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  CRD & 5000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  FS & 1000 & 0.10 (0.09, 0.10) & 0.03 (0.03, 0.04) \\ 
  FS & 3000 & 0.09 (0.09, 0.10) & 0.07 (0.06, 0.08) \\ 
  FS & 5000 & 0.10 (0.09, 0.10) & 0.08 (0.07, 0.09) \\ 
  HK & 1000 & 0.76 (0.68, 0.81) & 0.53 (0.40, 0.63) \\ 
  HK & 3000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  HK & 5000 & 1.00 (1.00, 1.00) & 1.00 (1.00, 1.00) \\ 
  SL & 1000 & 0.09 (0.08, 0.10) & 0.03 (0.02, 0.04) \\ 
  SL & 3000 & 0.08 (0.07, 0.09) & 0.06 (0.05, 0.07) \\ 
  SL & 5000 & 0.08 (0.06, 0.10) & 0.07 (0.05, 0.08) \\ 
   \hline
\end{tabular}
\caption{$F_1$ and ARI scores for various non-goal block sizes in SBM simulation 4. Parenthetical values are 5 and 95\% percentiles. Percentiles are taken across Monte Carlo Samples. 500 Monte Carlo samples were taken per setting of non-goal block size.} 
\label{tab:sbmSize}
\end{table}

